The Landau Collision Integral in the Particle Basis in the PETSc Library

The Landau collision integral is often considered the gold standard in the context of kinetic plasma simulation due to its conservative properties, despite challenges involved in its discretization. The primary challenge when implementing an efficient computation of this operator is conserving physical properties of the continuum equation when the system is discretized. Recent work has achieved continuum discretizations using the method of Finite Elements which maintain conservation of mass, momentum, and energy, but which lacks monotonic entropy production. More recently, a particle discretization has been introduced which conserves mass, momentum, and energy, but maintains the benefit of monotonic entropy production necessary for the metriplecticity of the system. We present here an implementation of the particle basis Landau collision integral in the Portable Extensible Toolkit for Scientific Computing in 2 and 3V for the construction of a full geometry solver with a novel approach to computation of the entropy functional gradients. Verification of the operator is achieved with thermal equilibration and isotropization tests. All examples are available, open source, in the PETSc repository for reproduction.

==> performance.tex <==
\section{Adaptive Time Stepping}
There exists a tradeoff of physcially meaning results versus precision in terms of how the time stepping is handled. Many small time steps acquire full conservation, however adaptive stepping achieves physical results with asymptotic behavior in the error of the second moment (energy). Adaptive time stepping is obviously fruitful as the largest time steps possible greatly reduce computational overhead, however, adaptivity remains challenging due to the stability region of the method. While conservation may be relatively controlled, convergence to the appropriate, equal final states in isotropization test cases remains challenging, with improper temperatures being reached by each species in their final states.
